Domain-invariant Feature Exploration for Domain Generalization

Deep learning has achieved great success in the past few years. However, the performance of deep learning is likely to impede in face of non-IID situations. Domain generalization (DG) enables a model to generalize to an unseen test distribution, i.e., to learn domain-invariant representations. In this paper, we argue that domain-invariant features should be originating from both internal and mutual sides. Internal invariance means that the features can be learned with a single domain and the features capture intrinsic semantics of data, i.e., the property within a domain, which is agnostic to other domains. Mutual invariance means that the features can be learned with multiple domains (cross-domain) and the features contain common information, i.e., the transferable features w.r.t. other domains. We then propose DIFEX for Domain-Invariant Feature EXploration. DIFEX employs a knowledge distillation framework to capture the high-level Fourier phase as the internally-invariant features and learn cross-domain correlation alignment as the mutually-invariant features. We further design an exploration loss to increase the feature diversity for better generalization. Extensive experiments on both time-series and visual benchmarks demonstrate that the proposed DIFEX achieves state-of-the-art performance.

==> sec-relatedwork-cikm.tex <==
% \section{Related Work}
\subsection{Domain generalization}
Existing domain generalization approaches~\cite{wang2021generalizing} mainly consists of data augmentation~\cite{shankar2018generalizing,tobin2017domain}, domain-invariant feature learning~\cite{muandet2013domain,ganin2016domain,li2018domain}, and meta-learning~\cite{li2018learning,balaji2018metareg} techniques.
Most of existing work pays attention to some specific application such as computer vision and reinforcement learning.
Our work belongs to domain-invariant feature learning-based DG, where we mainly focus on common domain-invariant feature learning methods which can be directly applied to different tasks.

% \subsection{Knowledge distillation}
% Knowledge distillation is a popular technique to effectively learn a student model from a teacher model. 
% It was proposed to train a small model to mimic a large model via logit matching~\cite{ba2014deep}.
% Various versions of distillation methods were proposed later.
% FITNETS~\cite{romero2014fitnets} tried to perform feature distillation for a small but deep network.
% \cite{komodakis2017paying} utilized the attention map as knowledge to transfer from teacher to student, which expected that students paid attention to the area that the teacher paid attention to.
% \cite{yim2017gift} defined the distilled knowledge to be transferred in terms of flow between layers, which was calculated by computing the inner product between features from two layers.
% Knowledge distillation makes a student model mimic a teacher model, and thereby these two models may share some similarities.

\subsection{Domain-invariant representations}

Domain-invariant representation learning~\cite{johansson2019support,ben2010theory} has long been a popular solution to addressing domain shift problems such as domain adaptation~\cite{ganin2015unsupervised,ganin2016domain,zhao2019learning} and domain generalization~\cite{li2018domain,muandet2013domain,matsuura2020domain}.
Specifically for DG, learning domain-invariant representations is critical since DG focuses on the invariance across domains.
Such domain invariance is achieved can be achieved by explicit feature alignment~\cite{li2018domain,motiian2017unified}, adversarial learning~\cite{ganin2016domain,li2018deep,rahman2020correlation}, or disentanglement~\cite{liu2020learning,peng2019domain,ilse2020diva}. 
Recently, some work pointed that only simple alignments maybe not enough for generalization~\cite{bui2021exploiting}.
Our work share the same goal with them, but with more possibilities to explore more invariant features that allows more diversities to increase the generalization ability.
Our framework may seem similar to the disentanglement framework from many existing efforts since it also learns two kinds of features and then combines them for final prediction.
However, it significantly differs from them since we are actually learning two kinds of domain-invariant features, while disentanglement often learns invariant and specific features.
%还有那个domain-invariant单独不太好的两篇文章

\subsection{Fourier features}
%还有新的那两篇的说明
Recently, several work paid attention to Fourier phase in visual recognition~\cite{yang2020fda,xu2021fourier}.
FDA~\cite{yang2020fda} introduced the Fourier perspective into domain adaptation.
It could generate target-like images for training via simply replacing a small area in the centralized amplitude spectrum of a source image with that of a target image.
FACT~\cite{xu2021fourier} illustrated that Fourier phase information contained high-level semantics and was not easily affected by domain shifts.
It utilized the mixup~\cite{zhang2018mixup} technique to enlarge the diversity of Fourier amplitude without changing labels and thereby learned a model that was insensitive to Fourier amplitude.
Another work~\cite{zhao2021testtime} utilized Fourier amplitude (style) to calibrate the target domain style on the fly. 
However, it required some operations when testing.
Some other work tried to control Fourier amplitude during training for better generalization~\cite{lin2022deep,zheng2022famlp}.
These work are designed for the visual field, although much work~\cite{oppenheim1979phase,oppenheim1981importance,hansen2007structural} have demonstrated that the phase component retains most of the high-level semantics in original signals, which suggests that Fourier phase may be a kind of universal domain-invariant features.
